Gaussian Process Morphable Models

Statistical shape models (SSMs) represent a class of shapes as a normal distribution of point variations, whose parameters are estimated from example shapes. Principal component analysis (PCA) is applied to obtain a low-dimensional representation of the shape variation in terms of the leading principal components. In this paper, we propose a generalization of SSMs, called Gaussian Process Morphable Models (GPMMs). We model the shape variations with a Gaussian process, which we represent using the leading components of its Karhunen-Loeve expansion. To compute the expansion, we make use of an approximation scheme based on the Nystrom method. The resulting model can be seen as a continuous analogon of an SSM. However, while for SSMs the shape variation is restricted to the span of the example data, with GPMMs we can define the shape variation using any Gaussian process. For example, we can build shape models that correspond to classical spline models, and thus do not require any example data. Furthermore, Gaussian processes make it possible to combine different models. For example, an SSM can be extended with a spline model, to obtain a model that incorporates learned shape characteristics, but is flexible enough to explain shapes that cannot be represented by the SSM. We introduce a simple algorithm for fitting a GPMM to a surface or image. This results in a non-rigid registration approach, whose regularization properties are defined by a GPMM. We show how we can obtain different registration schemes,including methods for multi-scale, spatially-varying or hybrid registration, by constructing an appropriate GPMM. As our approach strictly separates modelling from the fitting process, this is all achieved without changes to the fitting algorithm. We show the applicability and versatility of GPMMs on a clinical use case, where the goal is the model-based segmentation of 3D forearm images.

==> background.tex <==
%!TEX root = gpregistration.tex

\section{Gaussian Process basics}\label{sec:gp-basics}
In this section we quickly summarize in this section the main concepts related to Gaussian Processes, which we use in our method. 
\subsection{Gaussian processes}

Stochastic processes allow to define a probability distribution
over a function space.  Formally, a stochastic process is a collection
of random variables $f(x), x \in \Omega$ where $\Omega$ is an index
set. In particular, a Gaussian process is a stochastic process with the property
that for any finite number of observations, $x_1, \ldots, x_n \in
\Omega$ the values $f(x_1), \ldots, f(x_n)$ are jointly normally
distributed \cite{rasmussen_gaussian_2006}.  A Gaussian process is completely defined by a mean
$\mu : \Omega \to \R$ and a covariance function $k: \Omega \times \Omega
\to \R$.  We write $\GP(\mu, k)$ to specify a Gaussian process.  To
simplify the discussion, only Gaussian processes
$\GP(0, k)$ with zero mean are considered, the extension to the general case is,
however, straight-forward.

By choosing a covariance function $k(x,y)$, it is specifyed which functions are likely given this process. 
The covariance function defines for each pair of points $x, y$ their covariance
$E[f(x)f(y)]$. Moreover, covariance functions are often referred to as kernels, and we will use the
terms interchangeably.
For many known covariance functions nearby values are strongly correlated, which effectively leads to a preference of smooth functions. 
%Indeed, many covariance functions  
%arise as Greens functions of common regularization operators \cite{wahba_spline_1990}.
% The most well known in the registration community are the spline based kernels, such as
% those corresponding to B-splines or Elastic Body splines (TODO cite Elastic body spline, TODO define it?)
% Due to the popularity of Gaussian processes and kernel methods in the machine learning 
% community, many other covariance functions are known and well studied. 


\subsection{Vector-valued Gaussian Processes} \label{sec:vec-gp}
For modeling deformation fields using Gaussian processes, the above
concepts need to be generalized to vectorial random variables, where
$u(x)$ is $d$ dimensional.\footnote{While in the statistical
  literature, vector valued Gaussian processes are usually referred to
  as Gaussian Random fields, we will not make this distinction in this
  paper, and refer to the process as a Gaussian process, independently
  of the dimensionality.} Correspondingly, the covariance function,
becomes a matrix valued function $k(x,y) : \Omega \times \Omega \to
\R^{d \times d}$, with $k(x,y) = E[u(x)^Tu(y)]$.  It can be shown that
the vector-valued case can be reduced to the scalar case.  Thus all
known results for real-valued Gaussian processes carry over to this
more general setting. Further details can be found in Hein et al.\
\cite{hein_kernels_2004}.

% Hein et al. \cite{hein2004kas} showed that there is no need to extend the theory from the scalar case. 
% Instead, one can reduce the vector valued case to the scalar case by changing the domain of the problem to 
% $\Omega \times [1, \ldots, d]$ and considering the real-valued covariance function
%  \[
%  l: (\Omega \times [1,\ldots, d] ) \times (\Omega \times [1,\ldots, d]
%  ) \to \R
%  \]
% defined by 
% \[
% l((x,s), (y,t)) =  k_{st}(x,y).
% \]
A particular class of vector valued covariance functions  
arise from the scalar valued case. Let 
$A \in \mathbb{R}^{d \times d}$ be a symmetric, positive definite matrix and $l$ a
real valued covariance function. Then,
the matrix valued function $k$ with entries $k_{ij}$ defined by
 \begin{equation} \label{eq:fs:a-kernel}
   k_{ij}(x,y) = A_{ij} l(x,y), 
 \end{equation}
is a valid covariance function \cite{micchelli_learning_2005}. 
The entry $A_{ij}$ determines the correlation between the $i$-th and $j$-th output component.
In cases where no a-priori knowledge about their correlation is given, each dimension can be considered
as independent from the others by choosing $A = \mathcal{I}_{d}$ as being the identity.

\subsection{Mercer's expansion and reproducing kernel Hilbert spaces} \label{sec:mercer-expansion}
Closely related to a Gaussian process $\GP(\mu, k)$ is the reproducing kernel Hilbert space (RKHS) which is spanned by the covariance function $k$. A starting point to construct such a space is the eigenfunction expansion of $k$. According to 
Mercer's theorem (see e.g. \cite{rasmussen_gaussian_2006}), a positive definite kernel $k$ has an expansion in terms of a orthonormal set of basis functions:
\begin{equation} \label{eq:mercer}
k(x,y) = \sum_{i=1}^\infty \lambda_i \phi_i(x)\phi_i(y)^T , 
\end{equation}
where $(\lambda_i, \phi_i)$ are the eigenvalue/eigenfunctions pairs of the 
integral operator $
\mathcal{T}_k f(\cdot) := \int_\Omega k(x,\cdot) f(x) \, dp(x), 
$
where $dp(x)$ is a probability measure on $\Omega$. (TODO check that the rest of this section is consistent with this measure).
Linear combinations of these eigenfunctions: $f(x) = \sum_{i=1}^N  \phi_i(x) \alpha_i$ with $\sum_{i=1}^n \alpha_i^2/\lambda_i < \infty$ form a Hilbert space where the inner product between two functions  $f = \sum_{i=1}\alpha_i \phi_i$ and $g =
\sum_{j=1} \beta_j \phi_j$ is defined by 
$%\begin{equation}\label{eq:fs:dotprod-mercer}
\dotprod{f}{g}_k = \sum_{i=1}^\infty \frac{\alpha_i \beta_i}{\lambda_i}.
$
Hence, the norm becomes
\begin{equation} \label{eq:fs:mercer-rkhs-norm}
\norm{f}_k^2 = \dotprod{f}{f}_k = \sum_{i=1}^\infty \frac{\alpha_i^2}{\lambda_i}.
\end{equation}
Note that the RKHS norm is mainly influenced by eigenfunction components corresponding to small eigenvalues, a fact that is considered in Section~\ref{sec:reg-low-rank-model}. 

To close the circle, a Gaussian process can be defined in terms of this expansion. 
Let
\begin{equation} \label{eq:klt}
u(x) = \mu(x) + \sum_{i=1}^\infty \alpha_i \sqrt{\lambda_i}\phi_i(x), \; \alpha_i \in N(0, 1),
\end{equation}
which is equivalent to 
\[
u \sim GP(\mu, k).
\]

\subsection{Gaussian Process Regression} \label{sec:gp-regression}
Consider a given i.i.d. sample ${S} = \{(x_1, y_1,),
\ldots, (x_n, y_n)\} \subset \Omega \times \R^d$ and let $u \in \GP(0,
k)$ be a vector valued Gaussian process with $k: \Omega \times \Omega
\to \R^{d \times d}$.  Let us infer the distribution $p(u |S)$.
Additionally, lets assume that noisy instances $y \sim \mathcal{N}(u(x), \sigma^2
\mathcal{I}_d)$ of the actual values $u(x)$ are ovserved.
Then, the likelihood of the
data is given as
$
p({S} | u)  = \prod_{i=1}^n \mathcal{N}(u(x_i), \sigma_i).
$
Under this assumption the posterior distribution $p(u|{S}) \propto p(u) p({S}|u)$ is known in closed form \cite{rasmussen_gaussian_2006}. It is again a Gaussian process $\GP(\mu_p, k_p)$ and its parameters are 
 \begin{align}  \label{eq:gp-vec-post}
   \mu_p(x) &= K_X(x)^T (K_{XX} + \sigma^2\mathcal{I})^{-1}Y\\
   k_p(x,x') &= k(x, x') - 
   K_X(x)^T(K_{XX}+\sigma^2\mathcal{I})^{-1}K_X(x').
 \end{align}
 Here, we defined $K_X(x) = (k(x, x_i))_{i=1}^n \in \R^{nd \times
   d}$, $K_{XX} = \left(k(x_i, x_j)\right)_{i,j=1}^n \in \R^{nd \times nd}$ and $Y
 = (y_1, \ldots, y_n)^T \in \R^{nd}$. Note that $K_X$ and $K_{XX}$
 consist of sub-matrices of size $d \times d$.
 
 Given this posterior distribution, only functions that agree with the
 given sample ${S}$ are likely observations. This is
 illustrated in Figure~\ref{fig:gp-samples}.  Figure~\ref{fig:gp-samples-prior} shows random samples from a
 one-dimensional prior distribution where we used the Gaussian
 covariance function, defined by $k(x,x')= \exp(-\norm{x
   -x'}^2/4)$. Figure~\ref{fig:gp-samples-post} shows the corresponding
 posterior distribution after the sample has been observed. 
 % We note that all the samples agree with the given test
 % points, up to some small approximation error, that is determined by
 % the value of $\sigma^2$ that we use.  If we chose $\sigma^2 = 0$, all
 % solutions perfectly interpolate the training points.
 \begin{figure}[t]
   \subfloat[]{\includegraphics[width=0.5\columnwidth,height=2.5cm]{images/prior_samples} \label{fig:gp-samples-prior}}
   \subfloat[]{\includegraphics[width=0.5\columnwidth,height=2.5cm]{images/posterior_samples}\label{fig:gp-samples-post}}
 \caption{\protect \subref{fig:gp-samples-prior} Random samples from a Gaussian process. \protect \subref{fig:gp-samples-post} 
 Random samples from the posterior process, after a number of points have been observed. Only functions that agree with the observations are likely to be observed.}
 \label{fig:gp-samples}
 \end{figure}



%%% Local Variables: ***
%%% mode:latex ***
%%% TeX-master: "gpregistration.tex"  ***
%%% End: ***

